Learning from Censored and Dependent Data: The case of Linear Dynamics

Observations from dynamical systems often exhibit irregularities, such as censoring, where values are recorded only if they fall within a certain range. Censoring is ubiquitous in practice, due to saturating sensors, limit-of-detection effects, and image-frame effects. In light of recent developments on learning linear dynamical systems (LDSs), and on censored statistics with independent data, we revisit the decades-old problem of learning an LDS, from censored observations (Lee and Maddala (1985); Zeger and Brookmeyer (1986)). Here, the learner observes the state $x_t \in \mathbb{R}^d$ if and only if $x_t$ belongs to some set $S_t \subseteq \mathbb{R}^d$. We develop the first computationally and statistically efficient algorithm for learning the system, assuming only oracle access to the sets $S_t$. Our algorithm, Stochastic Online Newton with Switching Gradients, is a novel second-order method that builds on the Online Newton Step (ONS) of Hazan et al. (2007). Our Switching-Gradient scheme does not always use (stochastic) gradients of the function we want to optimize, which we call "censor-aware" function. Instead, in each iteration, it performs a simple test to decide whether to use the censor-aware, or another "censor-oblivious" function, for getting a stochastic gradient. In our analysis, we consider a "generic" Online Newton method, which uses arbitrary vectors instead of gradients, and we prove an error-bound for it. This can be used to appropriately design these vectors, leading to our Switching-Gradient scheme. This framework significantly deviates from the recent long line of works on censored statistics (e.g., Daskalakis et al. (2018); Kontonis et al. (2019); Daskalakis et al. (2019)), which apply Stochastic Gradient Descent (SGD), and their analysis reduces to establishing conditions for off-the-shelf SGD-bounds.

==> abstract.tex <==
We introduce the algorithm \emph{Mareva}. %The polynomial dependence on $n$ is much larger than $n^3$ (achieved for known cost function).


\ignore{

We study the control of an \emph{unknown} linear dynamical system under general convex costs. The objective we consider is regret with respect to stable linear policies. This generalizes the online linear quadratic regulator, where costs are convex quadratics. We build the first polynomial-time algorithm with $\sqrt{T}$-regret for the case where the cost function is known. To do so, we introduce a novel exploration strategy based on convex geometry. In particular, we adaptively construct a sequence of weak John ellipsoids to explore an over-parameterized policy space. Before our work, the best known regret bound was $T^{2/3}$ \cite{}.
\par
We also study control with bandit feedback, i.e., assuming the cost function is unknown. We design a second polynomial-time algorithm which applies to this more general setting and which also achieves $\sqrt{T}$-regret. In case the cost function is known, the first algorithm enjoys significantly better regret bounds in terms of the dimension dependence compared to the second one.
\par Finally, in accordance with previous works, we show that under strong assumptions, a simple method based on online gradient descent gives $\sqrt{T}$-regret, for known cost function.
\\
\\
{\color{red}Missing from intro, but not sure where to put: Motivation for considering linear policies for convex costs since they are suboptimal in general: for convex costs the optimal policies are very complex, i.e. piecewise linear with exponentially many parts in the worst case. So, linear policies until now have been used in all works for regret bounds as tractable baselines. We leave the important extension to larger policy classes for future work. }
}

==> maybe-trash.tex <==
\ref{eq:init-bounds} hold. From Theorem \ref{thm:init}, $\Pr[\neg \mE_0]\le o(1)$. Given $\mE_0$, we will establish the remaining conditions of Theorem \ref{thm:main}.
\par \op{move this paragraph to appdx}First, we show that $\mK$ is $R$-accurate with $R=\poly\left(\frac{1}{\alpha\beta}\right)\cdot \sqrt{d}$. On $\mE_0$, $\sA\in \mK$, and for all $t$, $\|x_t\|_{\Sigma_0^{-1}}\le \poly\left(\frac{1}{\alpha\beta}\right)\cdot \|x_t\|_{\ga_T^{-1}}.$ By unrolling the system, $x_t=\sum_{k=0}^{t-1}\sA^kw_{t-k-1}$, and so $x_t\sim \mN\left(0,\sum_{k=0}^{t-1}\sA^k{\left(\sA^k\right)}^T\right)$. Since $\ga_T\succcurlyeq \sum_{k=0}^{t-1}\sA^k{\left(\sA^k\right)}^T$, $\|x_t\|_{\ga_T^{-1}}=\|\ga_t^{-1/2}x_t\|$ is stochastically dominated by a $\|z\|$, where $z\sim \mN(0,I)$. So, from concentration of Gaussian norm (\cite{vershynin2018high}), $\|x_t\|_{\ga_T^{-1}}$ is $O(d)$-subgaussian.
\par Second, again from concentration of Gaussian norm, $\|w_t\|$ is $R_w^2$-subgaussian, with $R_w=O\left(\sqrt{d}\right)$. Third, for all $t$, we have $\Ex[\|x_t\|^2]=\trace{\left(\sum_{k=0}^{t-1}\sA^k{\left(\sA^k\right)}^T\right)}\le \trace(\ga_T)\coloneqq R_x^2$. In Appendix \ref{appdx:cl:gammaT}, we show that $\trace(\Gamma_T)=O\left(\frac{d}{1-\rho(\sA)}\cdot \text{cond}(U)^{2}\right)$ $(\text{remember}\ \sA=UDU^{-1})$. Let $\Sigma=\frac{1}{|I_1|}\sum_{t\in \mI_1}x_tx_t^T$. Having established all conditions of Theorem \ref{thm:time-series}, using Markov's inequality in \ref{eq:error-bound}, we have that with probability at least $1-\delta$, \footnote{Observe that our bounds depend on $1/\delta$. It is possible to achieve $\log{(1/\delta)}$ dependence, but with more technical proofs. To keep the presentation simpler, we chose not to optimize this dependence.}
\begin{align}\label{eq:markov-final}
    \|\whA-\sA\|_{\Sigma}^2&\le \tO(1)\cdot \frac{\poly({1/\alpha})}{\delta N}\left(d(d+R^2+R_w^2)+L(d+R^2+R_w^2)\right) \notag \\
    &\le \tO(1)\cdot \poly({1/\alpha}) \cdot\frac{d^2+dL}{\delta N}.
\end{align}
Now, on $\mE_0$, $\Sigma\succcurlyeq \ga_T/\poly(1/\beta)$. Also, from Proposition \ref{prop:largeN}, with probability at least $1-o(1)$, $N=|\mP_1|\ge |\mP|/2\ge \alpha \beta T/4$. So, for $\mE_{\text{num}}=\{N<\alpha\beta T/4\}$, we have $\Pr[\neg \mE_{\text{num}}]\le o(1)$. Choosing sufficiently small $\delta=\Omega(1)$, and letting $\mE_\text{b}$ be the event that the bound on $\|\whA-\sA\|_\Sigma^2$ in \ref{eq:markov-final} holds, we get $\Pr[\mE_0 \land \mE_{\text{num}} \land \mE_{\text{b}}]\ge 99\%$.
Observe that on $\mE_0 \land \mE_{\text{num}} \land \mE_{\text{b}}$, $\|\whA-\sA\|_{\ga_T}\le \tO(1)\cdot \poly\left(\frac{1}{\alpha\beta}\right)\cdot \sqrt{\frac{d^2+dL}{T}}$.
